A Retrieval-Based Approach to Medical Procedure Matching in Romanian

Accurately mapping medical procedure names from healthcare providers to standardized terminology used by insurance companies is a crucial yet complex task. Inconsistencies in naming conventions lead to missclasified procedures, causing administrative inefficiencies and insurance claim problems in private healthcare settings. Many companies still use human resources for manual mapping, while there is a clear opportunity for automation. This paper proposes a retrieval-based architecture leveraging sentence embeddings for medical name matching in the Romanian healthcare system. This challenge is significantly more difficult in underrepresented languages such as Romanian, where existing pretrained language models lack domain-specific adaptation to medical text. We evaluate multiple embedding models, including Romanian, multilingual, and medical-domain-specific representations, to identify the most effective solution for this task. Our findings contribute to the broader field of medical NLP for low-resource languages such as Romanian.

==> tables/combined.tex <==
\begin{table*}[hbt!]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lc|c|cccc}
        \textbf{Model Name} & \textbf{Index Type} & \textbf{Mode Type} & \textbf{Acc@1} & \textbf{Acc@3} & \textbf{Acc@5} & \textbf{Acc@100}\\
        \toprule
        RoBERT \cite{masala-etal-2020-robert} & \multirow{6}{*}{masterlist} & \multirow{3}{*}{off-the-shelf} & 44.7 $\pm$ 0.003 & 53.4 $\pm$ 0.003 & 56.9 $\pm$ 0.004 & 75.3 $\pm$ 0.003 \\
        BioClinicalBERT \cite{alsentzer2019clincalbert}  &  &  & 47.7 $\pm$ 0.003 & 56.7 $\pm$ 0.003 & 60.2 $\pm$ 0.002 & 74.9 $\pm$ 0.003\\
        mE5 \cite{wangMultilingualE5Text2024}  &  &  & 56.8 $\pm$ 0.003 & 69.4 $\pm$ 0.002 & 74.3 $\pm$ 0.002 & 91.3 $\pm$ 0.002\\
        %\midrule
        \cmidrule(l){3-7}
        RoBERT \cite{masala-etal-2020-robert} & & \multirow{3}{*}{fine-tuned} & 75.9 $\pm$ 0.001 & 89.9 $\pm$ 0.002 & 93.2 $\pm$ 0.000 & 98.9 $\pm$ 0.001\\
        BioClinicalBERT \cite{alsentzer2019clincalbert} &  & & 75.7 $\pm$ 0.002 & 89.2 $\pm$ 0.002 & 92.7 $\pm$ 0.002 & 98.9 $\pm$ 0.000\\
        mE5 \cite{wangMultilingualE5Text2024}  & &  &\textbf{ 78.8 $\pm$ 0.002} & \textbf{92.2 $\pm$ 0.002} & \textbf{95.0 $\pm$ 0.002} & \textbf{99.5 $\pm$ 0.001}\\
        \midrule
        RoBERT \cite{masala-etal-2020-robert} & \multirow{6}{*}{masterlist + mappings} & \multirow{3}{*}{off-the-shelf} & 62.5 $\pm$ 0.005 & 76.8 $\pm$ 0.004 & 81.1 $\pm$ 0.005 & 92.0 $\pm$ 0.004\\
        BioClinicalBERT \cite{alsentzer2019clincalbert} &  &  & 66.7 $\pm$ 0.005 & 80.8 $\pm$ 0.003 & 84.6 $\pm$ 0.002 & 93.4 $\pm$ 0.002\\
        mE5 \cite{wangMultilingualE5Text2024} &  &  & 67.9 $\pm$ 0.004 & 85.2 $\pm$ 0.002 & 89.6 $\pm$ 0.002 & 98.1 $\pm$ 0.001\\
        \cmidrule(l){3-7}
        RoBERT \cite{masala-etal-2020-robert} &  & \multirow{3}{*}{finetuned} & 84.4 $\pm$ 0.002 & 94.8 $\pm$ 0.002 & 96.6 $\pm$ 0.001 & 99.0 $\pm$ 0.001\\
        BioClinicalBERT \cite{alsentzer2019clincalbert} &  &  & 83.8 $\pm$ 0.003 & 94.3 $\pm$ 0.001 & 96.4 $\pm$ 0.001 & 99.0 $\pm$ 0.001\\
        mE5 \cite{wangMultilingualE5Text2024} &  & & \textbf{85.2 $\pm$ 0.003} & \textbf{95.8 $\pm$ 0.001} & \textbf{97.5 $\pm$ 0.001} & \textbf{99.5 $\pm$ 0.001}\\
    \end{tabular}
    }
    \caption{Comparison between different types of text embedding models, having entries in the vector store only from the masterlist entries. We obtained the best results using a fine-tuned version of mE5, a general-purpose multi-lingual model. Results are averaged across 5 folds.}
    \label{tab:masterlist}
\end{table*}
